A Robust Framework for Classifying Evolving Document Streams in an Expert-Machine-Crowd Setting

An emerging challenge in the online classification of social media data streams is to keep the categories used for classification up-to-date. In this paper, we propose an innovative framework based on an Expert-Machine-Crowd (EMC) triad to help categorize items by continuously identifying novel concepts in heterogeneous data streams often riddled with outliers. We unify constrained clustering and outlier detection by formulating a novel optimization problem: COD-Means. We design an algorithm to solve the COD-Means problem and show that COD-Means will not only help detect novel categories but also seamlessly discover human annotation errors and improve the overall quality of the categorization process. Experiments on diverse real data sets demonstrate that our approach is both effective and efficient.

==> 04-blocked_experiments.tex <==
% !TEX root = paper.tex

\begin{figure}[t]
%\centering
\includegraphics[width=\columnwidth]{figs/all_results_based_on_coh-v2}
\caption{Evaluation of the newly generated clusters in terms of their coherence\label{fig:coh.user_study}}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{figs/all_results_based_on_novelty-v2}
\caption{Evaluation of the newly generated clusters in terms of their novelty\label{fig:novelty.user_study}}
\end{figure}

\subsection{Coherence based evaluation of emerging clusters}
As in our case, one of the key requirements is to generate clusters which are highly coherent i.e. items within the newly generated cluster are very related to each other, in this experiment we aim to conduct a user study to ask crowd workers to determine the element of cohesiveness in our new clusters. For this purpose, we generate clusters using the settings described in the section~\ref{sec:baseline} i.e. we use $k_o+n+1$ clusters, where $k_o=5$, $n=4$ and the value found for $\ell$ in the previous experiment for each dataset is used.
%
Top $m$ (where $m=2$ in our case as explained above) largest coherent clusters are selected among the newly emerged clusters of the $Z$ category. Outliers are removed from the both selected clusters. Next, crowdsourcing tasks are generated using 10 pairs of randomly selected items from each cluster.

Workers on the Crowdflower platform were asked to read each pair of items and specify whether the items are very related, somewhat related, or not related to each other. Figure~\ref{fig:cf_task_for_coh_nov} shows the crowdsourcing task we designed for this purpose. Three judgments from 3 different workers were required to finalize a task (i.e. a pair of items in our case). The final answer for a pair is decided based on the majority voting technique. In this task the inter-annotator agreement was 74\%.

Figure~\ref{fig:coh.user_study} depicts the results obtained from the user study. ``very related'' and ``somewhat related'' values are much more common than ``not related,'' supporting the claim that the new clusters are perceived by users as containing items of the same topic.

% \usepackage{multirow}


\subsection{Novelty based evaluation of emerging clusters}
One of the required characteristics of the newly emerged clusters is their high novelty i.e. items in the new clusters must not be similar with the items in the existing clusters. To determine whether clusters emerged using our proposed technique are really novel or not, we conduct another user study. We generate clusters using the settings described in the section~\ref{sec:baseline} i.e. we use $k_o+n+1$ clusters, where $k_o=5$, $n=4$ and the optimal value of $\ell$  found in the previous experiment for each dataset.
%
Top $m$ (where $m=2$ in our case as explained above) largest novel clusters are selected among the newly emerged clusters of the $Z$ category. For each selected $N_i$ cluster, 10 items are randomly picked to form pairs with the items of the existing categories (i.e. clusters of $T_i$). One item of $N_i$ is paired with 10 items of $T_i$ clusters.

For each pair, workers were asked to indicate whether items in a pair are very related, somewhat related, or not related. Figure~\ref{fig:cf_task_for_coh_nov} shows the crowdsourcing task we used. Three judgments from 3 different workers were required to finalize a task. The final answer for a pair is decided based on the majority voting technique. In this task the inter-annotator agreement was 79\%.

Figure~\ref{fig:novelty.user_study} depicts the results obtained from the user study. We can see that most of the answers are ``Not related'' and some are ``somewhat related'', which indicates that the items in the new clusters are indeed different than the items in the existing categories.

